Globally Consistent Video Depth and Pose Estimation with Efficient Test-Time Training

Dense depth and pose estimation is a vital prerequisite for various video applications. Traditional solutions suffer from the robustness of sparse feature tracking and insufficient camera baselines in videos. Therefore, recent methods utilize learning-based optical flow and depth prior to estimate dense depth. However, previous works require heavy computation time or yield sub-optimal depth results. We present GCVD, a globally consistent method for learning-based video structure from motion (SfM) in this paper. GCVD integrates a compact pose graph into the CNN-based optimization to achieve globally consistent estimation from an effective keyframe selection mechanism. It can improve the robustness of learning-based methods with flow-guided keyframes and well-established depth prior. Experimental results show that GCVD outperforms the state-of-the-art methods on both depth and pose estimation. Besides, the runtime experiments reveal that it provides strong efficiency in both short- and long-term videos with global consistency provided.

==> tables/7scenes-new.tex <==
\begin{tabular}{lcR{1.1cm}R{1.1cm}R{1.1cm}R{1cm}R{1.1cm}R{1.3cm}R{1.3cm}}
\hline
\multicolumn{1}{c}{\multirow{3}{*}{Method}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}known\\ pose?\end{tabular}} & \multicolumn{4}{c}{Depth Metrics} & \multicolumn{3}{c}{Pose Metrics} \\
\multicolumn{1}{c}{} &  & \multirow{2}{*}{\tiny{AbsRel$\downarrow$}} & \multirow{2}{*}{\tiny{SqRel$\downarrow$}} & \multirow{2}{*}{\tiny{RMSE$\downarrow$}} & \tiny{$\delta<$} & \tiny{ATE} & \tiny{RPE Trans} & \tiny{RPE Rot} \\
\multicolumn{1}{c}{} &  &  &  &  & \tiny{$1.25\uparrow$} & \tiny{(m)$\downarrow$} & \tiny{(m) $\downarrow$} & \tiny{(deg) $\downarrow$} \\ \hline
DPSNet$\dagger$~\cite{im2019dpsnet} & \checkmark & 0.199 & 0.142 & 0.438 & 0.710 & - & - & - \\
CNMNet$\dagger$~\cite{long2020occlusion} & \checkmark & 0.161 & 0.083 & 0.361 & 0.766 & - & - & - \\
NeuralRecon$\dagger$~\cite{sun2021neuralrecon} & \checkmark & 0.155 & 0.104 & 0.347 & 0.820 & - & - & - \\ \hline
DeepV2D~\cite{teed2018deepv2d} &  & 0.162 & 0.092 & 0.380 & 0.767 & 0.471 & 1.018 & 60.979 \\
DROID-SLAM~\cite{teed2021droid} & \multicolumn{1}{l}{} & 0.209 & 0.132 & 0.462 & 0.665 & 0.463 & 0.928 & 40.143 \\ \hline
Deep3D~\cite{lee20213d} &  & 0.172 & 0.105 & 0.406 & 0.748 & 0.310 & 0.306 & 8.665 \\
CVD2~\cite{kopf2021robust} &  & 0.154 & 0.085 & 0.379 & 0.795 & 0.375 & 0.517 & 31.102 \\
Ours (GCVD) &  & \textbf{0.124} & \textbf{0.054} & \textbf{0.307} & \textbf{0.858} & \textbf{0.249} & \textbf{0.257} & \textbf{8.155} \\ \hline
\end{tabular}

==> tables/7scenes.tex <==
\begin{tabular}{l|c|cccc|rrr}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}known\\ pose?\end{tabular}} & \multicolumn{4}{c|}{Depth Metrics} & \multicolumn{3}{c}{Pose Metrics} \\
 &  & {Abs Rel$\downarrow$} & {Sq Rel$\downarrow$} & {RMSE$\downarrow$} & {$\delta<1.25\uparrow$} & \multicolumn{1}{c}{{ATE {(m)}$\downarrow$}} & \multicolumn{1}{c}{{RPE Trans {(m)}$\downarrow$}} & \multicolumn{1}{c}{{RPE Rot {(deg)}$\downarrow$}} \\ \hline
DPSNet$\dagger$~\cite{im2019dpsnet} & \checkmark & 0.199 & 0.142 & 0.438 & 0.710 & - & -\hspace{0.15cm} & -\hspace{0.3cm} \\
CNMNet$\dagger$~\cite{long2020occlusion} & \checkmark & 0.161 & 0.083 & 0.361 & 0.766 & - & -\hspace{0.15cm} & -\hspace{0.3cm} \\
NeuralRecon$\dagger$~\cite{sun2021neuralrecon} & \checkmark & 0.155 & 0.104 & 0.347 & 0.820 & - & -\hspace{0.15cm} & -\hspace{0.3cm} \\ \hline
DeepV2D~\cite{teed2018deepv2d} &  & 0.162 & 0.092 & 0.380 & 0.767 & 0.471 & 1.018\hspace{0.15cm} & 60.979\hspace{0.3cm} \\
Deep3D~\cite{lee20213d} &  & 0.172 & 0.105 & 0.406 & 0.748 & 0.310 & 0.306\hspace{0.15cm} & 8.665\hspace{0.3cm} \\
CVD2~\cite{kopf2021robust} &  & 0.154 & 0.085 & 0.379 & 0.795 & 0.375 & 0.517\hspace{0.15cm} & 31.102\hspace{0.3cm} \\
Ours &  & \textbf{0.124} & \textbf{0.054} & \textbf{0.307} & \textbf{0.858} & \textbf{0.249} & \textbf{0.257}\hspace{0.15cm} & \textbf{8.155}\hspace{0.3cm} \\ \hline
\end{tabular}

==> tables/ablation-new.tex <==
\begin{tabular}{C{1.4cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.4cm}C{1.4cm}}
\hline
\multicolumn{5}{c}{Ablation settings} & \multicolumn{2}{c}{Errors $\downarrow$} \\
\multirow{2}{*}{keyframe} & layer & mesh & grad. & \multirow{2}{*}{PGO} & \multicolumn{1}{c}{Depth} & \multicolumn{1}{c}{Pose} \\
 & norm & deform. & loss &  & \multicolumn{1}{c}{AbsRel} & \multicolumn{1}{c}{ATE} \\ \hline
\checkmark &  &  &  &  & 0.208 & 0.555 \\
\checkmark & \checkmark &  &  &  & 0.137 & 0.332 \\
\checkmark & \checkmark & \checkmark &  &  & 0.132 & 0.327 \\
\checkmark & \checkmark & \checkmark & \checkmark &  & 0.125 & 0.277 \\
 & \checkmark & \checkmark & \checkmark &  & 0.127 & 0.308 \\
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \textbf{0.124} & \textbf{0.249} \\ \hline
\end{tabular}

==> tables/ablation-rot.tex <==
\begin{tabular}{lcccccc}
\hline
keyframe & \checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark \\
layer normalization &  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
mesh deformation &  &  & \checkmark & \checkmark & \checkmark & \checkmark \\
depth gradient loss &  &  &  & \checkmark & \checkmark & \checkmark \\
pose graph optimization &  &  &  &  &  & \checkmark \\ \hline
Depth AbsRel $\downarrow$ & \multicolumn{1}{r}{0.208} & \multicolumn{1}{r}{0.137} & \multicolumn{1}{r}{0.132} & \multicolumn{1}{r}{0.125} & \multicolumn{1}{r}{0.127} & \multicolumn{1}{r}{\textbf{0.124}} \\
Pose ATE $\downarrow$ & \multicolumn{1}{r}{0.555} & \multicolumn{1}{r}{0.332} & \multicolumn{1}{r}{0.327} & \multicolumn{1}{r}{0.277} & \multicolumn{1}{r}{0.308} & \multicolumn{1}{r}{\textbf{0.249}} \\ \hline
\end{tabular}

==> tables/ablation.tex <==
\begin{tabular}{ccccccc}
\hline
\multicolumn{5}{c}{Ablation settings} & \multicolumn{2}{c}{Errors $\downarrow$} \\ \hline
\begin{tabular}[c]{@{}c@{}}\footnotesize{key-}\\ \footnotesize{frame}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\footnotesize{layer}\\ \footnotesize{norm}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\footnotesize{mesh}\\ \footnotesize{deform.}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\footnotesize{grad.}\\ \footnotesize{loss}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\footnotesize{loop}\\ \footnotesize{close}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\footnotesize{Depth}\\ \footnotesize{Abs Rel}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\footnotesize{Pose}\\ \footnotesize{ATE}\end{tabular} \\ \hline
\checkmark &  &  &  &  & \small{0.208} & \small{0.555} \\
\checkmark & \checkmark &  &  &  & \small{0.137} & \small{0.332} \\
\checkmark & \checkmark & \checkmark &  &  & \small{0.132} & \small{0.327} \\
\checkmark & \checkmark & \checkmark & \checkmark &  & \small{0.125} & \small{0.277} \\
 & \checkmark & \checkmark & \checkmark &  & \small{0.127} & \small{0.308} \\
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \textbf{\small{0.124}} & \textbf{\small{0.249}} \\ \hline
\end{tabular}

==> tables/euroc.tex <==
\begin{tabular}{lrrr}
\hline
Sequence & \multicolumn{1}{c}{Deep3D} & \multicolumn{1}{c}{CVD2} & \multicolumn{1}{c}{Ours} \\ \hline
\footnotesize{{\fontfamily{qcr}\selectfont MH\_01\_easy}} & 3.24 & 1.48 & \textbf{1.33} \\
\footnotesize{{\fontfamily{qcr}\selectfont MH\_02\_easy}} & 3.82 & \textbf{1.32} & 1.72 \\
\footnotesize{{\fontfamily{qcr}\selectfont MH\_03\_medium}} & 2.82 & 2.63 & \textbf{1.99} \\
\footnotesize{{\fontfamily{qcr}\selectfont MH\_04\_difficult}} & 4.26 & 4.20 & \textbf{3.78} \\
\footnotesize{{\fontfamily{qcr}\selectfont MH\_05\_difficult}} & 5.06 & \textbf{4.31} & 4.59 \\
\footnotesize{{\fontfamily{qcr}\selectfont V1\_01\_easy}} & 1.53 & \textbf{0.94} & 1.11 \\
\footnotesize{{\fontfamily{qcr}\selectfont V1\_02\_medium}} & 1.57 & 1.63 & \textbf{1.07} \\
\footnotesize{{\fontfamily{qcr}\selectfont V1\_03\_difficult}} & 1.32 & \textbf{1.19} & 1.33 \\
\footnotesize{{\fontfamily{qcr}\selectfont V2\_01\_easy}} & 1.97 & 1.43 & \textbf{0.96} \\
\footnotesize{{\fontfamily{qcr}\selectfont V2\_02\_medium}} & 1.87 & \textbf{1.56} & 1.88 \\
\footnotesize{{\fontfamily{qcr}\selectfont V2\_03\_difficult}} & 1.73 & 1.74 & \textbf{1.46} \\ \hline
\textbf{Mean} & 2.65 & 2.04 & \textbf{1.93} \\ \hline
\end{tabular}

==> tables/time.tex <==
\begin{tabular}{L{2.15cm}R{1.3cm}R{1.3cm}R{1.3cm}R{1.3cm}R{1.3cm}}
\hline
\# frames & 50 & 200 & 500 & 1000 & 2000 \\ \hline
CVD2~\cite{kopf2021robust} & 13.90 & 14.83 & 17.34 & 21.73 & 26.13 \\
Deep3D~\cite{lee20213d} & 4.13 & 3.03 & 2.75 & 2.66 & 2.61 \\
Ours (GCVD) & 2.40 & 2.53 & 2.74 & 2.83 & 3.04 \\ \hline
\end{tabular}

==> tables/tum-individual.tex <==
\begin{tabular}{l|ccccc|cccc}
\hline
\multirow{2}{*}{Sequence} & \multicolumn{5}{c|}{Pose Error (ATE in meters) $\downarrow$} & \multicolumn{4}{c}{Depth Error (Abs Rel) $\downarrow$} \\ \cline{2-10} 
 & \multicolumn{1}{c|}{COLMAP} & DeepV2D & Deep3D & CVD2 & Ours & DeepV2D & Deep3D & CVD2 & Ours \\ \hline
\notsotiny\texttt{fr1\_desk} & \multicolumn{1}{c|}{0.019} & 0.505 & 0.580 & 0.273 & \textbf{0.229} & 0.1440 & 0.1940 & 0.1090 & \textbf{0.0940} \\
\notsotiny\texttt{fr1\_desk2} & \multicolumn{1}{c|}{0.027} & 0.386 & 0.611 & 0.314 & \textbf{0.156} & 0.1679 & 0.2282 & \textbf{0.1139} & 0.1305 \\
\notsotiny\texttt{fr2\_desk} & \multicolumn{1}{c|}{0.818} & 0.331 & \textbf{0.260} & 0.613 & 0.422 & 0.1579 & \textbf{0.0973} & 0.1544 & 0.1130 \\
\notsotiny\texttt{fr3\_cabinet} & \multicolumn{1}{c|}{\textcolor{red}{failed}} & \textbf{0.220} & 1.225 & 0.444 & 0.850 & 0.1785 & 0.4613 & \textbf{0.1236} & 0.1832 \\
\notsotiny\texttt{fr3\_nstr\_tex\_near\_loop} & \multicolumn{1}{c|}{0.015} & 1.548 & 0.694 & 0.491 & \textbf{0.399} & 0.1516 & 0.2437 & 0.0615 & \textbf{0.0352} \\
\notsotiny\texttt{fr3\_sitting\_static} & \multicolumn{1}{c|}{0.033} & 0.018 & 0.006 & 0.029 & \textbf{0.006} & 0.2149 & 0.2368 & 0.1260 & \textbf{0.1243} \\
\notsotiny\texttt{fr3\_str\_tex\_far} & \multicolumn{1}{c|}{0.008} & 0.214 & \textbf{0.089} & 0.169 & 0.131 & 0.1476 & \textbf{0.0511} & 0.0742 & 0.0810 \\ \hline
Mean & \multicolumn{1}{c|}{0.153} & 0.460 & 0.495 & 0.333 & \textbf{0.313} & 0.1660 & 0.2160 & 0.1089 & \textbf{0.1087} \\ \hline
\end{tabular}

==> tables/tum-wilddepth.tex <==
\begin{tabular}{lR{1.1cm}R{1.1cm}R{1.1cm}R{1.2cm}R{1.2cm}R{1.5cm}R{1.5cm}}
\hline
\multirow{3}{*}{Method} & \multicolumn{4}{c}{Depth Metrics} & \multicolumn{3}{c}{Pose Metrics} \\
 & \multirow{2}{*}{{AbsRel$\downarrow$}} & \multirow{2}{*}{{SqRel$\downarrow$}} & \multirow{2}{*}{{RMSE$\downarrow$}} & {$\delta<$} & {ATE} & {RPE Trans} & {RPE Rot} \\
 &  &  &  & {$1.25\uparrow$} & {(m)$\downarrow$} & {(m) $\downarrow$} & {(deg) $\downarrow$} \\ \hline
\multicolumn{1}{l}{Gordon~\etal~\cite{gordon2019depth}} & 0.219 & 0.207 & 0.759 & 0.617 & 1.176 & 0.791 & 52.237 \\
\multicolumn{1}{l}{Ours} & \textbf{0.108} & \textbf{0.077} & \textbf{0.460} & \textbf{0.861} & \textbf{0.313} & \textbf{0.277} & \textbf{15.919} \\ \hline
\end{tabular}

==> tables/tum.tex <==
\begin{tabular}{l|cc|c}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{Depth} & Pose \\
 & \footnotesize{AbsRel$\downarrow$} & \footnotesize{$\delta<1.25\uparrow$} & \footnotesize{ATE$\downarrow$} \\ \hline
COLMAP~\cite{schonberger2016structure} & - & - &  \\
DeepV2D~\cite{teed2018deepv2d} & 0.1660 & 0.745 & 0.460 \\
Deep3D~\cite{lee20213d} & 0.2160 & 0.686 & 0.495 \\
CVD2~\cite{kopf2021robust} & 0.1089 & \textbf{0.887} & 0.333 \\
Ours & \textbf{0.1087} & 0.858 & \textbf{0.313} \\ \hline
\end{tabular}

==> tables/tum_simple.tex <==
\begin{tabular}{l|C{1.3cm}C{1.1cm}C{1.1cm}C{1.45cm}|C{1.15cm}C{1.15cm}C{1.45cm}}
\hline
\multirow{2}{*}{Sequence} & \multicolumn{4}{c|}{Pose Error (ATE in meters) $\downarrow$} & \multicolumn{3}{c}{Depth Error (Abs Rel) $\downarrow$} \\ \cline{2-8} 
 & \multicolumn{1}{c|}{COLMAP} & Deep3D & CVD2 & Our GCVD & Deep3D & CVD2 & Our GCVD \\ \hline
\texttt{fr1\_desk} & \multicolumn{1}{c|}{0.019} & 0.580 & 0.273 & {\ul 0.229} & 0.1940 & 0.1090 & {\ul 0.0940} \\
\texttt{fr1\_desk2} & \multicolumn{1}{c|}{0.027} & 0.611 & 0.314 & {\ul 0.156} & 0.2282 & {\ul 0.1139} & 0.1305 \\
\texttt{fr2\_desk} & \multicolumn{1}{c|}{0.818} & {\ul 0.260} & 0.613 & 0.422 & {\ul 0.0973} & 0.1544 & 0.1130 \\
\texttt{fr3\_cabinet} & \multicolumn{1}{c|}{\textcolor{red}{failed}} & 1.225 & {\ul 0.444} & 0.850 & 0.4613 & {\ul 0.1236} & 0.1832 \\
\texttt{fr3\_nstr\_tex\_near\_loop} & \multicolumn{1}{c|}{0.015} & 0.694 & 0.491 & {\ul 0.399} & 0.2437 & 0.0615 & {\ul 0.0352} \\
\texttt{fr3\_sitting\_static} & \multicolumn{1}{c|}{0.033} & 0.006 & 0.029 & {\ul 0.006} & 0.2368 & 0.1260 & {\ul 0.1243} \\
\texttt{fr3\_str\_tex\_far} & \multicolumn{1}{c|}{0.008} & {\ul 0.089} & 0.169 & 0.131 & {\ul 0.0511} & 0.0742 & 0.0810 \\ \hline
Mean & \multicolumn{1}{c|}{0.153} & 0.495 & 0.333 & \textbf{0.313} & 0.2160 & 0.1089 & \textbf{0.1087} \\ \hline
\end{tabular}
